Do Transformer Attention Heads Provide Transparency in Abstractive Summarization?

Learning algorithms become more powerful, often at the cost of increased complexity. In response, the demand for algorithms to be transparent is growing. In NLP tasks, attention distributions learned by attention-based deep learning models are used to gain insights in the models' behavior. To which extent is this perspective valid for all NLP tasks? We investigate whether distributions calculated by different attention heads in a transformer architecture can be used to improve transparency in the task of abstractive summarization. To this end, we present both a qualitative and quantitative analysis to investigate the behavior of the attention heads. We show that some attention heads indeed specialize towards syntactically and semantically distinct input. We propose an approach to evaluate to which extent the Transformer model relies on specifically learned attention distributions. We also discuss what this implies for using attention distributions as a means of transparency.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	samples/sample-manuscript.tex \
	samples/sample-acmsmall.tex \
	samples/sample-acmlarge.tex \
	samples/sample-acmtog.tex \
	samples/sample-sigconf.tex \
	samples/sample-authordraft.tex \
	samples/sample-xelatex.tex \
	samples/sample-sigplan.tex \
	samples/sample-sigchi.tex \
	samples/sample-sigchi-a.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

samples/%: %
	cp $^ samples

samples/sample-acmsmall.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmsmall]{acmart}/' $< > $@

samples/sample-acmlarge.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmlarge,screen]{acmart}/' $< > $@

samples/sample-acmtog.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmtog]{acmart}/' $<   > $@

samples/sample-sigconf.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigconf]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-authordraft.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigconf,authordraft]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-xelatex.tex: samples/sample-sigconf.tex
	cp $< $@

samples/sample-sigplan.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigplan,screen]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-sigchi.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigchi]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-sigchi-a.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigchi-a]{acmart}/' $< | \
	sed 's/begin{figure}\[h\]/begin{marginfigure}/' | \
	sed 's/end{figure}/end{marginfigure}/' | \
	sed 's/begin{table}/begin{margintable}/' | \
	sed 's/end{table}/end{margintable}/'   > $@


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut

distclean: clean


#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf samples/sample-*.pdf *.cls *.bst


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
		Font changes for SIGCHI table captions


Version 1.56    Bug fixes
		Added \flushbottom to two column formats (Philip Quinn)
		The final punctuation for the list of concepts
		is now period instead of semilcolon (Philip Quinn)
		New command \Description to describe images for visually
		impaired users.

Version 1.57    Change of \baselinestretch now produces an error
		Booktabs is now always loaded
		Added option `balance' to balance last page in two-column mode
		E-mail is no longer split in addresses
		New samples (Stephen Spencer)

==> old_introduction.tex <==

% \begin{itemize}
%     \item (0,1) Mostly to same summary word [timestep]
%     \item (0,3) Mostly same summary word [timestep]
%     \item (0,5) Attends previously generated word [timestep]
%     \item (0,6) ADP, in, on, with, of [overall]
%     \item (1,3) Attends previously generated word [timestep]
%     \item (1,2) Key words [overall]
%     \item (1,4) Mostly punctuation (full stop), but per time step it seems to focus on either full stops or everything but full stops.
%     \item (1,5) Entities, 'said','told', [overall]
%     \item (1,7) Seems to focus at locations [overall]
%     \item (2,1) Entities/days [overall]
%     \item (2,6) Attends to same word as summary word [timestep]
%     \item (3,0) Points to word of summary [both]
%     \item (3,5) Comma's quotes and random stuff [overall]
% \end{itemize}


% \begin{itemize}
%     \item 
%     \item Attention is commonly used as interpretability tool (cite ~2 papers) because it 'looks good', but: 1) a lot of 'contextual computation' happens between the input tokens and the hidden states that attention weights operate on, 2) examples are usually cherry picked, and 3) Attention is not Explanation paper.
%     \item Introduce Transformer as 'modular'/'disentangled' model (cite blog post on parallel to capsule networks?)
%     \item We investigate the multi-headed attention distribution for all layers for the encoder and decoder for transformers in a qualitative and quantitative way. In our qualitative settings we find that some heads consistently attend to locations, persons, nouns, verbs or punctuation. We investigate this more quantitatively by introducing several metrics.
%     \item  Our proposed adversarial attention
% \end{itemize}


% In recent years the attention mechanism \cite{bahdanau2014neural, luong2015effective} has gained popularity in the research community \todo{cite work}. Often the behaviour of the attention mechanism is used to achieve some insight in the behaviour of the model under consideration \todo{cite}. \citet{jain2019attention} recently argued that `attention is not explanation', by showing that different attention distributions can lead to the same output. \citeauthor{jain2019attention} only considered \todo{XXX} type of models and did not consider sequence-to-sequence architectures. In this work we look into the attention distributions of transformer models \cite{vaswani2017attention} that we train for the textual summarization task. Specifically we look into the cross-attention distributions. We investigate whether we can interpret those distributions and how they differ over different model initializations. To get even more insight in the behaviour of the cross-attention distributions we argue that we need to adopt a similar approach as in \citet{jain2019attention}. Therefore we propose to extend their approach to the sequence-to-sequence task, specifically to a sequence-to-sequence task where a transformer architecture is used.


% Recent advances in sequence to sequence models have given rise to a new model class that competes with Recurrent Neural Networks and Convolutional Neural Networks. This \textit{Transformer} architecture, introduced by \citet{vaswani2017attention}, is based solely on multi-headed (self) attention and eliminates the need for recurrency or convolutions.Attention is a mechanism that has been widely adopted in Natural Language Processing (NLP) models after being proposed by \citet{bahdanau2014neural,luong2015effective} in 2014 and 2015. Beside performance gains, attention is intuitively appealing and commonly interpreted as what a model focuses on for a given prediction \todo{MtH: Sources}. Although attention does provide a weight distribution over the input sequence based on a scoring function, this does not necessarily imply it should be interpreted as what the model is paying attention to \todo{MtH: Motivate this statement.}. With an increased focus on attention-based models as well as a growing demand for interpretability in complex deep learning models, it is important to understand what attention actually learns and how it effects an outcome.\todo{JB: Mention the underlying assumption that the attention weight for an encoder hidden state actually corresponds to the token at that location, even though this is questionable at least}

% This work aims to shed light on what multi-headed attention in a Transformer architecture learns when trained for abstractive summarization. Abstractive summarization is an interesting task because it requires a deep understanding of both the text as well as language in general. A good summarization model is thus expected to have an understanding of intermediate linguistic tasks, such as part of speech tagging and named entity recognition. We hypothesize that these linguistic patterns are learned in attention heads of the Transformer and investigate whether this can be quantitatively measured. We first adopt the visualization tool from \citet{see2017get} to be compatible with the multi-headed attention of a Transformer model. We then develop several metrics to quantify the intuition gained from the visualization tool. Finally, to investigate whether attention heads that seem to specialize towards linguistic tasks actually affect the predicted summary as expected, adversarial attacks on these attention heads are performed, following recent work by \citet{jain2019attention}.\\
%     \item Attention is commonly used as interpretability tool (cite ~2 papers) because it 'looks good', but: 1) a lot of 'contextual computation' happens between the input tokens and the hidden states that attention weights operate on, 2) examples are usually cherry picked, and 3) Attention is not Explanation paper.
%     \item Introduce Transformer as 'modular'/'disentangled' model (cite blog post on parallel to capsule networks?)
%     \item We investigate the multi-headed attention distribution for all layers for the encoder and decoder for transformers in a qualitative and quantitative way. In our qualitative settings we find that some heads consistently attend to locations, persons, nouns, verbs or punctuation. We investigate this more quantitatively by introducing several metrics.
%     \item  Our proposed adversarial attention
% \end{itemize}


% In recent years the attention mechanism \cite{bahdanau2014neural, luong2015effective} has gained popularity in the research community \todo{cite work}. Often the behaviour of the attention mechanism is used to achieve some insight in the behaviour of the model under consideration \todo{cite}. \citet{jain2019attention} recently argued that `attention is not explanation', by showing that different attention distributions can lead to the same output. \citeauthor{jain2019attention} only considered \todo{XXX} type of models and did not consider sequence-to-sequence architectures. In this work we look into the attention distributions of transformer models \cite{vaswani2017attention} that we train for the textual summarization task. Specifically we look into the cross-attention distributions. We investigate whether we can interpret those distributions and how they differ over different model initializations. To get even more insight in the behaviour of the cross-attention distributions we argue that we need to adopt a similar approach as in \citet{jain2019attention}. Therefore we propose to extend their approach to the sequence-to-sequence task, specifically to a sequence-to-sequence task where a transformer architecture is used.


% Recent advances in sequence to sequence models have given rise to a new model class that competes with Recurrent Neural Networks and Convolutional Neural Networks. This \textit{Transformer} architecture, introduced by \citet{vaswani2017attention}, is based solely on multi-headed (self) attention and eliminates the need for recurrency or convolutions.Attention is a mechanism that has been widely adopted in Natural Language Processing (NLP) models after being proposed by \citet{bahdanau2014neural,luong2015effective} in 2014 and 2015. Beside performance gains, attention is intuitively appealing and commonly interpreted as what a model focuses on for a given prediction \todo{MtH: Sources}. Although attention does provide a weight distribution over the input sequence based on a scoring function, this does not necessarily imply it should be interpreted as what the model is paying attention to \todo{MtH: Motivate this statement.}. With an increased focus on attention-based models as well as a growing demand for interpretability in complex deep learning models, it is important to understand what attention actually learns and how it effects an outcome.\todo{JB: Mention the underlying assumption that the attention weight for an encoder hidden state actually corresponds to the token at that location, even though this is questionable at least}

% This work aims to shed light on what multi-headed attention in a Transformer architecture learns when trained for abstractive summarization. Abstractive summarization is an interesting task because it requires a deep understanding of both the text as well as language in general. A good summarization model is thus expected to have an understanding of intermediate linguistic tasks, such as part of speech tagging and named entity recognition. We hypothesize that these linguistic patterns are learned in attention heads of the Transformer and investigate whether this can be quantitatively measured. We first adopt the visualization tool from \citet{see2017get} to be compatible with the multi-headed attention of a Transformer model. We then develop several metrics to quantify the intuition gained from the visualization tool. Finally, to investigate whether attention heads that seem to specialize towards linguistic tasks actually affect the predicted summary as expected, adversarial attacks on these attention heads are performed, following recent work by \citet{jain2019attention}.\\

